Convergence rates and approximation results for SGD and its continuous-time counterpart

This paper proposes a thorough theoretical analysis of Stochastic Gradient Descent (SGD) with non-increasing step sizes. First, we show that the recursion defining SGD can be provably approximated by solutions of a time inhomogeneous Stochastic Differential Equation (SDE) using an appropriate coupling. In the specific case of a batch noise we refine our results using recent advances in Stein's method. Then, motivated by recent analyses of deterministic and stochastic optimization methods by their continuous counterpart, we study the long-time behavior of the continuous processes at hand and establish non-asymptotic bounds. To that purpose, we develop new comparison techniques which are of independent interest. Adapting these techniques to the discrete setting, we show that the same results hold for the corresponding SGD sequences. In our analysis, we notably improve non-asymptotic bounds in the convex setting for SGD under weaker assumptions than the ones considered in previous works. Finally, we also establish finite-time convergence results under various conditions, including relaxations of the famous {\L}ojasiewicz inequality, which can be applied to a class of non-convex functions.

==> optimal_strongly.tex <==
\subsection{Quantitative constants in the strongly convex setting}
\label{sec:dependency-constant}


We first state a specific version of \Cref{lemma:ode} in the case
where there exists $t_0 > 0$ such that for any $t \geq 0$ and
$F(t, x) \geq -\rmf(x) \rmg(t)$ with $\rmf$ superlinear.

\begin{lemma_colt}
  \label{lemma:ode_plus}
  Let $F \in \rmc^1(\bR_+\times \bR, \bR)$ and
  $v \in \rmc^1(\bR_+,\bR_+)$ such that for all $t \geq 0$,
  $\rmd v(t)/\rmd t \leq F(t,v(t))$. Assume that there exist
  $\rmf: \ \rset \to \rset$, 
  $\rmg \in \rmc(\rset_+, \rset_+)$, $t_0 >0$,
  $A \geq 0$ and $\upbeta >0$ such that the following conditions hold.
  \begin{enumerate}[label=(\alph*)]
  \item \label{item:a_opt} For any $t \geq t_0$, $r \in \ocint{0, 1}$ and $u \geq 0$, $r F(t,u) \leq F(t, ru)$.
  \item \label{item:b_opt} For any $t \geq t_0$ and $u \geq 0$, $F(t,u) \leq -\rmf(u) \rmg(t)$.
  \item \label{item:c_opt} For any $u \geq A$, $\rmf(u) > \upbeta u$.
  \end{enumerate}
  Then, for any $t \geq 0$,
  \begin{equation}
    v(t) \leq \max\defEnsLigne{A, \exp[\upbeta(G(t_0) -G(t))]\max_{s \in \ccint{0, t_0}}v(s)} \eqsp,
    \end{equation}
    with $G(t) = \int_0^t \rmg(s) \rmd s$.
\end{lemma_colt}

\begin{proof}
  Let $T \geq 0$ and $v_T(t) = v(t) \exp[\upbeta(G(t) - G(T))]$. Using
  condition \ref{item:a_opt} and that $G$ is
  non-decreasing since for any $t \geq 0$, $\rmg(t) \geq 0$, we have
  for any $t \in \ocint{0,T}$
  \begin{equation}
    \rmd v_T(t) / \rmd t \leq \exp[\upbeta(G(t) - G(T))] F(t, v(t)) + \upbeta \rmg(t) v_T(t) \leq F(t, v_T(t)) + \upbeta \rmg(t) v_T(t) \eqsp .
  \end{equation}
  Using this result and conditions \ref{item:b_opt}-\ref{item:c_opt},
  we have for any $t \geq t_0$ such that $v_T(t) \geq A$
  \begin{equation}
    \label{eq:ineq_yT}
     \rmd v_T(t) / \rmd t \leq -\rmf(v_T(t)) \rmg(t) + \upbeta v_T(t) \rmg(t) < 0 \eqsp .
   \end{equation}
   Let $B = \max(A, \max_{s \in \ccint{0,t_0}} v_T(s))$. Assume that
   $\msa = \ensembleLigne{t \in \ccint{0,T}}{v_T(t) > B} \neq \emptyset$
   and let $t_1 = \inf \msa$. Note that $t_1 \geq t_0$ and
   $v_T(t_1) \geq A$. Therefore, using \eqref{eq:ineq_yT} we have
   $ \rmd v_T(t_1) / \rmd t < 0$ and therefore, there exists
   $0 < t_2 < t_1$ such that $v_T(t_2) > v_T(t_1)$ but then
   $t_2 \in \msa$ and $t_2 < \inf \msa$. Hence, $\msa = \emptyset$ and
   we get that for any $t \in \ccint{0,T}$, $v_T(t) \leq B$, % .
   % Therefore, we get that for any $t \geq 0$,
   % \begin{equation}
   %   v(t) = v_t(t) \leq \max\defEnsLigne{A, \exp[\upbeta(G(t_0) - G(t))] \max_{s \in \ccint{0,t_0}} v(s)} \eqsp ,
   % \end{equation}
   which concludes the proof.
\end{proof}

\begin{theorem}
	\label{prop:constante}
	Let $\alpha, \gamma \in \ooint{0,1}$ and $(\bfX_t)_{t\geq0}$ be given by
        \eqref{eq:sde}.  Assume \rref{assum:f_lip}, \rref{assum:grad_sto},
        \rref{assum:lip_sigma} and \rref{assum:strongly_cvx}. Then  for any $T \geq 0$,
        \begin{equation}
          \expeLigne{\norm{\bfX_T-x\st}^2} \leq \max \defEns{4 \gua \eta / \mu, C \expeLigne{\normLigne{\bfX_0 - x^{\star}}^2} \exp[-\mu (\gua + T)^{1-\alpha}/(2-2\alpha)]} ( \gua + T)^{-\alpha} \eqsp ,
        \end{equation}
        with
        \begin{equation}
          C = (1 + \eta \Psi(\alpha, t_0)) \exp[\mu (\gua +
t_0)^{1-\alpha}/(2-2\alpha)](\gua + t_0)^{\alpha} \eqsp .
        \end{equation}

\end{theorem}

\begin{proof}
  Let $\alpha, \gamma \in \ocint{0,1}$ and consider $\mce : \rset_+ \to \rset_+$
  defined for $t \geq 0$ by
  $\mce(t) = \expeLigne{(t+\gua)^{\alpha} \normLigne{\bfX_t - x^{\star}}^2}$,
  with $\gua = \gamma^{1/(1-\alpha)}$.  Using Dynkin's formula, see
  \Cref{lemma:dynkin}, we have for any $t\geq 0$,
\begin{align}
  \mce(t)=\mce(0) + \alpha \int_0^t  \frac{\mce(s)}{s+\gua}\dd s   + \int_0^t \gua \frac{\expe{\trace (\Sigma(\bfX_s))}}{ (s+\gua)^{\alpha}} \dd s -2 \int_0^t \expe{\la \nabla f(\bfX_s), \bfX_s-x\st \ra} \dd s
           \eqsp . \label{eq:strong_ito}
\end{align}
We now differentiate this expression with  respect to $t$ and
using \Cref{assum:strongly_cvx} and \Cref{assum:grad_sto}, we get for any $t > 0$,
\begin{align}
\rmd   \mce(t)/\rmd t &=\alpha \mce(t)(t+\gua)^{-1} -2 \expe{\la \nabla f(\bfX_t), \bfX_t-x\st \ra} + \gua \expe{\trace (\Sigma(\bfX_t))} (t+\gua)^{-\alpha} \\
  &\leq \alpha \mce(t)/(t+\gua) -2\mu \expeLigne{\normLigne{\bfX_t-x\st}^2} + \gua \eta/ (t+\gua)^{\alpha} \\
  &\leq F(t,\mce(t)) = \alpha \mce(t)(t+\gua)^{-1} -2\mu \mce(t)(t+\gua)^{-\alpha} + \gua \eta (t+\gua)^{-\alpha} \eqsp,
\end{align}
where we have used in the penultimate line that
$\trace(\Sigma(x)) \leq \eta$ for any $x \in \rset^d$ by
\Cref{assum:grad_sto}. Let
$t_0 = \max((\alpha/\mu)^{1/(1-\alpha)}-\gua, \gua)$. We have for any $t \geq t_0$, and $u \geq 0$
\begin{equation}
  F(t,u) \leq -\rmf(u) \rmg(t) \eqsp, \qquad \rmg(t) = (t+ \gua)^{-\alpha} \eqsp , \qquad \rmf(u) =\mu u - \gua \eta \eqsp .
\end{equation}
Hence the conditions \ref{item:a_opt} and \ref{item:b_opt} of
\Cref{lemma:ode_plus} are satisfied.  Let $\upbeta = \mu/2$ and
$A = 4 \gua \eta / \mu$. We obtain that for any $t \geq t_0$ and
$u \geq A$, $\rmf(u) > \mu u / 2$ and therefore condition
\ref{item:c_opt} of \Cref{lemma:ode_plus} is satisfied. Applying
\Cref{lemma:ode_plus}, we obtain that for any $t \geq 0$
\begin{equation}
  \mce(t) \leq \max( 4 \gua \eta / \mu, \exp[-\mu (\gua + t)^{1-\alpha}/(2-2\alpha)] B) \eqsp ,
\end{equation}
with
$B = \exp[\mu (\gua + t_0)^{1-\alpha}/(2-2\alpha)] \max_{s \in
  \ccint{0,t_0}} \mce(s)$.  We have that
$\max_{s \in \ccint{0,t_0}} \mce(s) \leq (t_0 + \gua)^{\alpha} \max_{s
  \in \ccint{0,t_0}} \expeLigne{\normLigne{\bfX_s -
    x^{\star}}}^2$. Using Dynkin's formula, see \Cref{lemma:dynkin},
we have for any $t\geq 0$,
\begin{equation}
  \expe{\norm{\bfX_t- x^{\star}}}^2 \leq \expe{\norm{\bfX_0- x^{\star}}}^2 + \eta \Psi(\alpha, t_0) \eqsp ,
\end{equation}
with
\begin{equation}
  \Psi(\alpha, t_0) =  \left \lbrace
  \begin{aligned}
    & \gamma^2 / (2\alpha - 1) & \text{if $2\alpha >1$ } \eqsp , \\
    & \gua \log(\gua^{-1} (t_0 + \gua))& \text{if $2\alpha = 1$ } \eqsp , \\
    & \gua (t_0 + \gua)^{1-2\alpha}/(1 - 2\alpha) & \text{otherwise} \eqsp .
  \end{aligned}
  \right.
\end{equation}
We conclude the proof upon setting
$C = (1 + \eta \Psi(\alpha, t_0)) \exp[\mu (\gua +
t_0)^{1-\alpha}/(2-2\alpha)](\gua + t_0)^{\alpha}$.
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main_colt"
%%% End:


==> trash.tex <==

\begin{wrapfigure}{R}{.4\textwidth}
  \begin{center}
    \scalebox{.6}{
		\begin{tikzpicture}[domain=0:1]
			\begin{axis}
        [
        ,axis equal,
        ,axis x line=bottom
  			,axis y line=center
				,ylabel near ticks,
				,xlabel near ticks,
        ,width=9cm
        ,xlabel=$\alpha$
        ,xmin=0
        ,xmax=1
        ,ymin=0
        ,ymax=1.1
        %,scaled ticks=true
        ,xtick={0,0.33,0.5,0.67,1}
        ,xticklabels={$0$,$1/3$,$1/2$,$2/3$,$1$},
        ,ytick={0,0.25,0.33,0.5,1},
        ,yticklabels={$0$,$1/4$,$1/3$,$1/2$,$1$}
        ,legend columns=2
        ,legend style={
        	at={(0.55,1.3)},
        	anchor=north,
        	/tikz/column 2/.style={
                column sep=5pt,
            }
        	}
        ]
        \addplot[solid][domain=0:0.5]{x} ;
        \addlegendentry{convex (Thm~\ref{thm:shamir_continuous})} ;
        \addplot[densely dashdotted][domain=0.5:1]{x} ;
        \addlegendentry{strongly convex} ;
        \addplot[loosely dashed][domain=0:0.5]{1-x} ;
        \addlegendentry{deterministic} ;
        \addplot[line width=1.2pt][domain=0.67:1]{1-x} ;
        \addlegendentry{Cor.\ref{cor:let-alpha-gamma}-\ref{item:a_weak}} ;
        \addplot[dashed, line width=1.2pt][domain=0:0.5]{x/2} ;
        \addlegendentry{Cor.\ref{cor:let-alpha-gamma}-\ref{item:b_weak}} ;
        %\addplot[dotted, line width=1.2pt][domain=0:0.33]{x/2} ;
        %\addlegendentry{Cor.\ref{cor:let-alpha-gamma}-\ref{item:c_weak}} ;
        \addplot[dotted][domain=0.5:0.67]{2*x-1} ;
        \addlegendentry{\citepalias{orvieto2019continuous}} ;

        \addplot[line width=1.2pt][domain=0.33:0.5]{3*x/2-1/2} ;
        \addplot[smooth][domain=0.5:0.67]{1-x} ;
        \addplot[line width=1.2pt][domain=0.5:0.67]{x/2} ;
    \end{axis}
  \end{tikzpicture}
  }
	\end{center}
	%\vspace*{-0.4cm}
	\caption{Comparison of the convergence rates obtained in the continuous case, against the results of~\citep{orvieto2019continuous} in the strongly convex, convex and weakly quasi convex settings. \label{fig:rates}}
	\vspace*{-1em}
\end{wrapfigure}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

